Handbook on Leveraging Lines for Two-View Relative Pose Estimation

We propose an approach for estimating the relative pose between calibrated image pairs by jointly exploiting points, lines, and their coincidences in a hybrid manner. We investigate all possible configurations where these data modalities can be used together and review the minimal solvers available in the literature. Our hybrid framework combines the advantages of all configurations, enabling robust and accurate estimation in challenging environments. In addition, we design a method for jointly estimating multiple vanishing point correspondences in two images, and a bundle adjustment that considers all relevant data modalities. Experiments on various indoor and outdoor datasets show that our approach outperforms point-based methods, improving AUC@10$^\circ$ by 1-7 points while running at comparable speeds. The source code of the solvers and hybrid framework will be made public.

==> 040.tex <==
\begin{tikzpicture}

  \draw[black, thick] (0,0) -- (1.5,0.2) -- (2.2,1.6) -- (0.6,1.3) -- (0,0);
  \draw[red, very thick] (0.2,0.2) -- (1.45,0.5)
  \draw[red, very thick] (0.3,0.5) -- (0.5,0.6)

\end{tikzpicture}

==> 500.tex <==
\begin{tikzpicture}
  \filldraw[blue] (0,0) circle (2pt);
  \filldraw[blue] (0.5,-0.8) circle (2pt);
  \filldraw[blue] (1.4,-0.6) circle (2pt);
  \filldraw[blue] (1.5,0.4) circle (2pt);
  \filldraw[blue] (0.7,0.7) circle (2pt);

\end{tikzpicture}

==> fig_latex/noise_orthogonality_test.tex <==
\begin{figure}
    \centering
    \setlength\tabcolsep{0pt}
    \setlength\extrarowheight{-3pt}
    \renewcommand{\arraystretch}{0}
    %\setlength\tabcolsep{0pt}
    \includegraphics[width=0.48\linewidth]{Figs/orth_legend.png}
    \begin{tabular}{c c}
       \includegraphics[width=0.43\linewidth]{Figs/ort_R.png}
       &
       \includegraphics[width=0.43\linewidth]{Figs/ort_t.png}
       \\
       %\includegraphics[width=0.45\linewidth]{Figs/ref_ort_R.png}
       %&
       %\includegraphics[width=0.45\linewidth]{Figs/ref_ort_t.png}
       %\\
    \end{tabular}
    
    \caption{
    \textbf{Angular error in deg. of solvers 2-1-1$^{\perp}$ and 1-2-1$^{\perp}$} (Fig.~\ref{fig:solvers_overview}) averaged over 100000 runs, as a function of deviation from the orthogonal direction. Results are without LO. 
    Image noise (i) and line number per VP (l/VP) are in the titles.
    %\todo{Write down this orthogonal noise in the the text.}
    %\todo{Orthogonal to Orthogonality}
    %\textbf{Study of the effect of deviation from the orthogonal direction on the result of the solvers assuming orthogonality}: The plots show how the rotation and the translation error depend on the deviation from the orthogonal direction. For every level of noise, we report a mean value over $100000$ samples. First row: without LO, second row: with LO.
    }
    \label{fig:noise_orthogonality_test}
\end{figure}


==> latex/abstract_v0.tex <==
Directly solving for the relative pose of 2 views from 2D line-to-line correspondences is impossible \PH{I don't think this word should appear in the first sentence of abstract. Also, this fact is very-well known, so we should not make it look as our contribution.} as they impose no explicit constraints.

As the main contribution, we propose ways of leveraging line matches in calibrated relative pose estimation.

To do so, we design five new minimal solvers that, together with point correspondences, exploit line coincidences: junctions, vanishing points, and coplanar lines.
%

We prove that the constraints implied by coplanar lines are equivalent to using line junctions, while the latter formulation leads to more stable solvers. 
%
    
Moreover, we propose a way for finding corresponding vanishing points jointly. % from line matches. 
%
We combine the proposed and existing solvers in a hybrid RANSAC framework to simultaneously benefit from lines, points and vanishing points.  
%
The methods are tested both on synthetic scenes, and on indoor and outdoor real-world datasets. 
%
The proposed hybrid approach is consistently superior to the state-of-the-art in terms of accuracy.


==> latex/conclusion_v0.tex <==

In this paper, we propose a number of new ways of leveraging 2D line-to-line correspondences to estimate the relative pose in two images. 
The proposed solvers, when combined with existing ones in a hybrid manner, lead to results superior to the state-of-the-art in terms of accuracy both indoors and outdoors on a number of datasets.
%
Moreover, the proposed joint vanishing point detection improves the VP-based solvers significantly.
Other algorithms, \eg performing auto-calibration, can also benefit from this method.
%
We believe that the accuracy can further be improved with a better line matcher or with a reliable algorithm to decide which line junctions refer to an underlying real 3D point -- this boils down to deciding which lines are coplanar.
%
We will make the source code of the hybrid estimator and the proposed solvers publicly available.



==> latex/intro_v0.tex <==
% General introduction of the problem that we solve
Finding the relative pose between a pair of images is a fundamental problem both in computer vision and robotics with a number of important real-world applications, \eg, 3D reconstruction \cite{DBLP:journals/cacm/AgarwalFSSCSS11, DBLP:conf/cvpr/BarathMESM21, DBLP:conf/cvpr/HeinlySDF15, DBLP:conf/cvpr/SchonbergerF16, DBLP:conf/cvpr/ZhuZZSFTQ18, DBLP:journals/ijcv/SnavelySS08}, visual localization \cite{DBLP:journals/ijrr/LynenZABHPSS20, DBLP:conf/eccv/PanekKS22, DBLP:conf/eccv/SattlerLK12, DBLP:conf/cvpr/SattlerMTTHSSOP18}, simultaneous localization and mapping \cite{DBLP:journals/corr/DeToneMR17, superpoint, DBLP:conf/eccv/EngelSC14, DBLP:journals/trob/Mur-ArtalMT15}, multi-view stereo \cite{DBLP:conf/iccv/ChenHXS19, DBLP:conf/cvpr/FurukawaCSS10, DBLP:journals/ftcgv/FurukawaH15, DBLP:conf/nips/KarHM17}, and visual odometry \cite{DBLP:conf/cvpr/NisterNB04, DBLP:journals/jfr/NisterNB06}.
%
% Estimating the relative pose is usually done from point correspondences found in the images. 
In this paper, we focus on estimating the relative pose leveraging both 2D line matches and point correspondences.
This allows being robust to various indoor and outdoor scene characteristics, \eg, low-textured areas where lines tend to be more distinctive than points.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth,trim={0 0 65mm 0},clip]{Figs/teaser3.pdf}
    \caption{\textbf{Relative pose from points and lines.} We propose to combine point, line, and vanishing point correspondences into a hybrid RANSAC~\cite{fischler1987} framework to recover the relative pose between two images. Our approach can handle typical failure cases of point-only solvers~\cite{DBLP:conf/cvpr/Nister03}, \eg in low textured areas.}
    \label{fig:teaser}
\end{figure}


% This is, to the best of our knowledge, has not yet been solved. 

% The traditional approach and its problems
The traditional approach for estimating the relative pose between two images starts with detecting \cite{SIFT2004, DBLP:conf/nips/RevaudSHW19, DBLP:conf/nips/TyszkiewiczFT20, superpoint} and matching \cite{sarlin20superglue} local features to form tentative point correspondences.
The points usually stem from corners or salient regions enabling to find the same features in multiple views in a repeatable manner. 
These matches are then usually fed into a robust estimator, \eg RANSAC~\cite{fischler1987} or one of its recent variants \cite{chum2003locally, DBLP:conf/cvpr/BarathNIM20, barath2018graph, DBLP:journals/pami/RaguramCPMF13, DBLP:conf/iccv/IvashechkinBM21}, in order to simultaneously find both the sought relative pose and the matches consistent with it. 
%
Even though this point-based approach is still a cornerstone of vision applications, it has certain weaknesses deteriorating its accuracy when the scene is dominated by homogeneous or repetitive regions. 
This is especially true in indoor environments \cite{7scenes, dai2017scannet, Schops_2017_eth3d} that tend to contain a large number of low-textured areas preventing to find strong features.
Also, repetitive structures often appear in man-made environments, \eg windows on a facade, breaking the visual descriptor-based feature matching.  


% Alternatives ways from e.g. other kinds of features like SIFT/AC and its problems
There are several other ways of estimating relative pose, either by using optical flow \cite{DBLP:journals/ai/HornS81, DBLP:conf/iccv/DosovitskiyFIHH15} or features containing richer information than only the point coordinates \cite{DBLP:journals/tip/BarathH18,barath2022relative}. 
%
While algorithms based on optical flow are widely used, \eg in SLAM pipelines \cite{DBLP:journals/trob/Mur-ArtalMT15}, they require the camera motion to be reasonably small.
Therefore, such approaches are not applicable to general relative pose estimation, where the cameras can move arbitrarily between the views.
%
Other algorithms exploit rich features, \eg affine correspondences, in order to solve the problem from fewer matches than when using only points.
This reduces the combinatorics of the robust estimation problem, thus often improving both the accuracy and the run-time. 
However, these methods suffer from the same issue as points: to find the affine shape accurately, the features must lie on salient regions \cite{HesHarAff2004, AffNet2018, Mishkin2015MODS, DBLP:journals/ipol/YuM11}.
Thus, they inevitably fail in low-textured environments.
\PH{Up to here, I don't see any problem.}

% Using lines for things
Using lines is known to be robust in indoor scenes \cite{7scenes, dai2017scannet, Schops_2017_eth3d}, for example, when performing 3D localization \cite{abdellali2021l2d2,gao2021pose} or reconstruction using 2D-3D line matches \cite{DBLP:journals/cviu/BartoliS05,zuo2017robust,pumarola2017pl,gomez2019pl,wei2019real,lim2021avoiding,shu2022structure}.
%
However, corresponding lines do not impose constraints on relative pose estimation~\cite{DBLP:conf/iccv/DuffKLP19} when having two views.
In the stereo case, their usage is limited to estimating the homography matrix via the well-known linear solver~\cite{guerrero2001lines}.
%
Since lines are particularly robust in certain scenarios, a number of papers investigate their usage when having more than two images~\cite{DBLP:conf/iccv/DuffKLP19, DBLP:conf/eccv/DuffKLP20, DBLP:conf/cvpr/FabbriDFRPTWHGK20, breiding2022line, Geppert2020ECCV, Geppert2021CVPR, DBLP:conf/cvpr/HrubyDLP22}.
%
% However, the run-times of such solvers (around one second) are unbearably high in practical applications. 
%
%Even though this homography can be decomposed to rotation and translation in the calibrated case, 
%
%\todo{Daniel: find and check out this paper.}
%
\PH{Reformulate from "There are no solvers." to "The solvers are not used (in the pipelines)." And add the CVPR 2011 paper. The rest seems OK.} The lack of two-view solvers stem from two issues.
First, 2D-2D line correspondences do not impose direct constraints on the pose.
Second, line matching is a particularly complicated problem, especially outdoors.
Until recently, there had been no reliable methods for detecting and matching lines both indoors and outdoors.

In this paper, we focus on investigating ways to leverage line-to-line correspondences for relative pose estimation in the calibrated two-view setting. 
%
To do it in a robust manner, we jointly exploit both point matches and line coincidences, \eg junction and vanishing point correspondences, and coplanar lines.
%
\PH{The following part until the end of the paragraph has to be completely changed.} \todo{We are the first to give a complete list of calibrated relpose minimal problems using pts, VPs and lines orthogonal to them. We design solvers to the problems from the list that have not been solved. We are the first to combine those solvers in a Hybrid RANSAC manner, and to show that using lines can be useful in practice, and lead to SOTA results. Also, we give the algorithm from 3rd contribution, and the LO.}
As the \textit{first} contribution, we propose five new minimal solvers simultaneously using multiple types of geometric entities.
As a \textit{second} contribution, we prove that the constraint derived from coplanar lines is actually equivalent to using line junctions, while leading to more stable solvers.
%
As the \textit{third} contribution, we develop an algorithm for finding vanishing point correspondences directly from line matches. 
%
As the \textit{fourth} contribution, the proposed solvers are combined together with well-known existing point-based ones, like the five-point algorithm~\cite{STEWENIUS2006284}, in a hybrid RANSAC framework to allow benefiting from all data types simultanously. 

The algorithms are tested both in a synthetic environment and on a number of real-world indoor and outdoor datasets \cite{7scenes, dai2017scannet, Schops_2017_eth3d, Jin2020}.
In the proposed hybrid framework, they always lead to results superior to the state-of-the-art in terms of accuracy while having comparable run-times. 


==> latex/local_optimization.tex <==
Following the common practice in RANSAC, we also apply local optimization in our hybrid RANSAC framework. Specifically, when a new best model is found, we apply the local optimization on randomly sampled subsets of the inliers for multiple times~\cite{Lebeda2012BMVC}. For point correspondences, we optimize the Sampson distance \cite{DBLP:books/cu/HZ2004}. For vanishing point correspondences, instead of optimizing the rotation directly over the input vanishing points, we combine the previously mentioned vanishing point optimization. In our optimization, each vanishing point is considered a dummy variable parameterized with a 3-dimensional homogeneous coordinate, which is constrained by both the line-VP distance from the 2D association and the sine value between the two directions after applying the relative rotation. Both the Sampson error and the vanishing point errors are combined together in a least square optimization via the Ceres solver \cite{ceres}, leading to a reliable estimation of the best relative pose model. 


==> latex/method_backup.tex <==
\noindent
In this section, we design multiple minimal solvers allowing to estimate the calibrated relative pose between two images from 2D line correspondences.
The proposed solvers are simultaneously using various types of geometric entities, like line, point, and vanishing point correspondences.
Point correspondences can stem from either line junctions \cite{DBLP:conf/cvpr/ElqurshE11}, endpoints, or from an off-the-shelf local feature detector and matcher, \eg, SuperPoint~\cite{superpoint} with SuperGlue~\cite{sarlin20superglue}. 
Vanishing points are extracted from the set of detected line matches prior to the relative pose estimation procedure. 

\input{fig_latex/solvers}

\subsection{Theoretical Background}

\noindent
Here, we describe the theoretical concepts used in the paper.

\textbf{Projection matrix} $\Proj_i \in \RR^{3\times4}$ of the $i$-th camera is decomposed as $\Proj_i = \Intrinsic_i [\Rot_i \ \Tran_i]$, where $\Intrinsic_i \in \RR^{3\times3}$ is the intrinsic matrix, and $\Rot_i \in \text{SO}(3), \Tran_i \in \RR^3$ represent the rotation and translation.
%
In case of having calibrated cameras, the projection matrix can be simplified to $\Proj_i = [\Rot_i \ \Tran_i]$.

\textbf{Relative pose} $(\Rot, \Tran)$ between two cameras $\Proj_1, \Proj_2$ is obtained as $\Rot = \Rot_2 \Rot_1^\text{T}$, $\Tran = \Tran_2 - \Rot_2 \Rot_1^\text{T} \Tran_1$.
%
The \textbf{epipolar geometry} \cite{DBLP:books/cu/HZ2004} relates the relative pose $(\Rot, \Tran)$ and a homogeneous 2D point correspondence $(\Point, \Point') \in \RR^3 \times \RR^3$ (PC). Let $\Worldpoint \in \RR^3$ be a point in space, $\Point$ be its projection into $\Proj_1$, and $\Point'$ be its projection into $\Proj_2$. 
Projections $\Point, \Point'$ are related by the epipolar constraint \cite{DBLP:books/cu/HZ2004} as ${\Point'}^\text{T} \Fund \Point = 0$,
%
%\begin{equation*}
%    {\Point'}^\text{T} \Fund \Point' = 0,
%\end{equation*}
%
where $\Fund$ is a fundamental matrix relating $\Proj_1$, $\Proj_2$. If the cameras are calibrated, the constraint is simplified to ${\Point'}^\text{T} \Ess \Point = 0$,
%
%\begin{equation*}
%    {\Point'}^\text{T} \Ess \Point' = 0,
%\end{equation*}
where $\Ess$ is the essential matrix relating cameras $\Proj_1$, $\Proj_2$. The essential matrix $\Ess$ is decomposed as $[\Tran]_{\times} \Rot$. Then, the epipolar constraint is written as
%
\begin{equation}
    {\Point'}^\text{T} [\Tran]_{\times} \Rot \Point = 0 \label{eq:epipolar_pts}.
\end{equation}
%
Equation \eqref{eq:epipolar_pts} imposes one constraint on the relative pose $\Rot, \Tran$. Since scale cannot be observed, the relative pose has 5 degrees of freedom, and it can be estimated from 5 point correspondences \cite{DBLP:conf/cvpr/Nister03}.

\textbf{Homography} relates planes projected into cameras $\Proj_1$, $\Proj_2$. 
Let $\Plane$ be a 3D plane, and $\Worldpoint \in \Plane$ be a point on plane $\Plane$. 
Its projections $\Point$, $\Point'$ into $\Proj_1$, $\Proj_2$ are related by
%
%\begin{equation}
    $\Point' \sim \Hom \Point$,
%\end{equation}
%
where $\Hom \in \RR^{3\times3}$ depends only on $\Proj_1$, $\Proj_2$, and $\Plane$.
%
Similarly, let $\Worldline_1 \subset \Plane$ be a line in its implicit form on plane $\Plane$. 
Its projections $\Line$, $\Line'$ into $\Proj_1$, $\Proj_2$ are related by
%
\begin{equation}
    \Line \sim \Hom^\text{T} \Line' \label{eq:hom_line}.
\end{equation}
%
We can estimate $\Hom$ from 4 coplanar line correspondences (LC) \cite{DBLP:books/cu/HZ2004}. 
% If cameras $\Proj_1$, $\Proj_2$ are calibrated, we can decompose $\Hom$ into $\Hom = \Rot - \Tran \Normline^\text{T}$ where $\Rot, \Tran$ is the relative pose and $\Normline$ is the normal of $\Plane$. \cite{20.500.11850/63639}.

\textbf{Vanishing point (VP)} is an intersection of projections of parallel lines. The homogeneous coordinates of the vanishing point $\Vanishing_i$ in camera $j$ are expressed as $\Vanishing_i \sim \Intrinsic_j \Rot_j \Dir_i,$
%
%\begin{equation*}
%    \Vanishing_i \sim \Intrinsic_j \Rot_j \Dir_i,
%\end{equation*}
%where $\Intrinsic_j \in \RR^{3\times3}$ is the matrix of camera intrinsics, $\Rot_j \in \text{SO}(3)$ is the rotation of the $j$-th camera, and 
where $\Dir_i \in \RR^3$ is the direction of the $i$-th line in 3D. If the camera is calibrated, then this formula is simplified as
%
\begin{equation}
    \Vanishing_i \sim \Rot_j \Dir_i \label{eq:VP_calibrated}.
\end{equation}
%
Let us have 2 calibrated cameras $\Proj_1 = [\Rot_1 \ \Tran_1]$, $\Proj_2 = [\Rot_2 \ \Tran_2]$. Vanishing points $\Vanishing$ in $\Proj_1$, $\Vanishing'$ in $\Proj_2$ are related by
%
\begin{equation}
    \Vanishing'  \sim \Rot_2 \Rot_1^\text{T} \Vanishing = \Rot \Vanishing \label{eq:van_sim},
\end{equation}
%
where $\Rot = \Rot_2 \Rot_1^\text{T} \in \text{SO}(3)$ is the relative rotation between $\Proj_1$, $\Proj_2$. Note that, if $\Vanishing$, $\Vanishing'$ are normalized, there must hold:
%
\begin{equation}
    \begin{split}
        \Vanishing' = \Rot \Vanishing \quad  \text{or} \quad \Vanishing' = -\Rot \Vanishing.
    \end{split} \label{eq:vanishing}
\end{equation}
%
One vanishing point correspondence (VC) gives two constraints on rotation $\Rot$. Two VCs fully determine $\Rot$. A third VC does not give additional constraints on the relative pose. See the supplementary material for details. 
%(See \ref{sec:third_vanishing} in the Supplementary material for details.) %Therefore, we consider minimal solvers using 0, 1, and 2 vanishing points.
\\

\subsection{Possible Configurations}
%
Considering the constraints described in the previous section, the number of distinct configurations of points, vanishing points, and lines orthogonal to them for estimating the relative pose is limited.
For their summary, see Fig.~\ref{fig:solvers_overview}. 
All other configurations can be traced back to these or do not provide additional constraints for relative pose.

\input{tab_latex/solver_overview}

~\\
\noindent
\textbf{Discussions on the completeness.}
We give here a high-level explanation that the list of configurations is complete. A full proof is given in Sec.~A in supp.
%
The relative pose has 5 degrees of freedom (DoF) \cite{DBLP:conf/cvpr/Nister03}.
%
The possible configurations can only have $0$, $1$, or $2$ VPs:
%
while $1$VP fixes 2DoF (Sec.~\ref{sec:2vp2pt}), and 2VP fix 3DoF (Sec.~\ref{sec:1vp3pt}), a third VP does not provide any additional constraints (see Sec. A in supp.).
Additionally, one line orthogonal to a VP can be used to create a second VP \cite{DBLP:conf/cvpr/ElqurshE11}; in the case of 2 VPs, a line orthogonal to one of them does not add any new information.

A point correspondence fixes 1 DoF \cite{DBLP:books/cu/HZ2004}. Four coplanar points fix 5 DoF due to the homography constraint \cite{DBLP:books/cu/HZ2004}. $n<4$ points are always coplanar, thus their coplanarity does not add any new constraints. 

We used these facts to obtain the possible configurations of points, vanishing points, and lines orthogonal to them.
Overall, the configurations can be clustered into 5 categories, summarized in Table~\ref{tab:configurations}.

~\\
\noindent
\textbf{Obtaining all configurations.}
To obtain more configurations, points can be replaced by lines with the following rules, where we adopt the solver notations of Fig. \ref{fig:solvers_overview}:
%
\begin{itemize}[noitemsep]
    \item 3 PCs can be replaced by \textit{3 coplanar lines}. Configuration 2-3-0 can thus be obtained from 5-0-0, and configuration 0-3-1 from 3-0-1.
    \item If we have 4 coplanar points, we can replace each of them with a line \cite{DBLP:books/cu/HZ2004}. Thus, the 4-0-0 configuration yields four new ones: 3-1-0, 2-2-0, 1-3-0, 0-4-0.
    \item One PC can be replaced with an intersection of two lines.    
    We prove in Sec.~B of supp. that using constraints implied by coplanar lines is equivalent to using their junctions as corresponding points. Therefore, 2-0-1$^{\perp}$, 2-1-1$^{\perp}$, and 1-2-1$^{\perp}$ belong to the same category.
\end{itemize}


All in all, the 5 categories of Table \ref{tab:configurations} yield the 13 configurations of Fig. \ref{fig:solvers_overview}.


\subsubsection{Existing Solvers}\label{sec:existing}

Some of the previously listed problems have already been solved.
Such configurations are the 5 PC solver~\cite{DBLP:conf/cvpr/Nister03, DBLP:conf/icpr/LiH06, STEWENIUS2006284, DBLP:conf/bmvc/KukelovaBP08}, the 4 PC, 4 LC, and combined homography solvers \cite{DBLP:books/cu/HZ2004}, and the 2-1-1$^{\perp}$ solver \cite{DBLP:conf/cvpr/ElqurshE11}. 2-3-0 is solved by 5PC solver. %Configuration 2-3-0 can be solved by 5 PC solver~\cite{DBLP:conf/cvpr/Nister03} after replacing the junctions with points. 
These we use as off-the-shelf solvers in our experiments.
%
In the next sections, we are deriving the proposed minimal solvers for the other investigated configurations.



\subsubsection{Pose from 1VC and 3PCs (3-0-1)}\label{sec:1vp3pt}

%\todo{Petr: replace the solver text}
%\todo{Petr: replace stability experiment with the new solver}
%\todo{Petr: add the solver to the C++ code}
%\todo{Daniel: re-run real experiments when Petr is done}
% \todo{Shaohui: chirality test}
%\todo{Shaohui: code cleaning + commenting}

Here, we are going to discuss how to calculate the relative pose $\Rot$, $\Tran$ from one vanishing point correspondence and three point correspondences.
%
Suppose that we are given a vanishing point match $(\Vanishing, \Vanishing')$, and three point correspondences $(\Point_1, \Point_1')$, $(\Point_2, \Point_2')$, $(\Point_3, \Point_3')$ in the two images, all normalized by the intrinsic camera matrices.


First, we are going to use the vanishing point to constrain rotation $\Rot$. The corresponding vanishing points are related by \eqref{eq:vanishing} which provides two systems of equations $\Vanishing'_1 = \Rot \Vanishing_1$ and $-\Vanishing'_1 = \Rot \Vanishing_1$.
If $\Rot \in \text{SO}(3)$ is a valid rotation matrix, it satisfies at least one of these systems. Each one is of form
%
\begin{equation}
    \mathbf{x}' = \Rot \mathbf{x}, \label{eq:13_general}
\end{equation}
%
where $\lVert \mathbf{x} \rVert = \lVert \mathbf{x}' \rVert = 1$. The task of estimating $\Rot$ and $\Tran$ with a constraint in form \eqref{eq:13_general} is similar to estimating the pose with known gravity \cite{DBLP:journals/jmiv/KalantariHJG11, DBLP:conf/eccv/FraundorferTP10, DBLP:conf/3dim/SweeneyFT14}.
%
We can resolve the sign ambiguity by checking the order of the lines, from which the VP was obtained. Based on \eqref{eq:13_general}, we can decompose $\Rot$ as follows:
%
\begin{equation}
    \Rot = {\Rot'}_{\mathbf{x}}^\text{T} \Rot_y \Rot_{\mathbf{x}}, \label{eq:13_rot_decomposition}
\end{equation}
%
where $\Rot_{\mathbf{x}}$ is a rotation that brings vector $\mathbf{x}$ to $y$-axis, ${\Rot}_{\mathbf{x}}'$ brings $\mathbf{x}'$ to $y$-axis, and $\Rot_y$ is rotation around the $y$-axis.

Let $\mathbf{b}_2 = [0 \ 1 \ 0]^\text{T}$ denote the $y$-axis direction. We find rotation $\Rot_{\mathbf{x}}$ using the Rodrigues formula as
%
\begin{equation*}
    \Rot_{\mathbf{x}} = \textbf{I} + \sin \alpha_x [\mathbf{a}_\mathbf{x}]_{\times} + (1-\cos \alpha_x) [\mathbf{a}_\mathbf{x}]_{\times}^2,
\end{equation*}
%
where $\alpha_x = \arccos \mathbf{x}^\text{T} \mathbf{b}_2$ is the angle between vector $\mathbf{x}$ and the $y$-axis, and $\mathbf{a}_\mathbf{x} = (\mathbf{x} \times \mathbf{b}_2) / \lVert \mathbf{x} \times \mathbf{b}_2 \rVert$ is the normalized cross product of $\mathbf{x}$ and the $y$-axis. We find rotation ${\Rot}_{\mathbf{x}}'$ in an analogous way.

Now, we are going to find rotation $\Rot_y$ and translation $\Tran$ from the point correspondences. From \eqref{eq:epipolar_pts}, there holds
%
\begin{equation}
    {\Point'_i}^\text{T} [\Tran]_{\times} {\Rot'}_{\mathbf{x}}^\text{T} \Rot_y(\varphi) \Rot_{\mathbf{x}} {\Point_i} = 0, \ i \in \{1,2,3\}, \label{eq:13_epipolar}
\end{equation}
%
where
\begin{equation*}
    \Rot_y(\varphi) = \begin{bmatrix}
        \cos \varphi & 0 & -\sin \varphi\\
        0 & 1 & 0\\
        \sin \varphi & 0 & \cos \varphi\\
    \end{bmatrix}.
\end{equation*}
The essential matrix $[\Tran]_{\times} {\Rot'}_{\mathbf{x}}^\text{T} \Rot_y(\varphi) \Rot_{\mathbf{x}}$ from \eqref{eq:13_epipolar} is equal to ${\Rot'}_{\mathbf{x}}^\text{T} [\Tran']_{\times} \Rot_y(\varphi) \Rot_{\mathbf{x}}$ where $\Tran' = {\Rot'}_{\mathbf{x}} \Tran$. We calculate $\Qoint_i = \Rot_{\mathbf{x}} \Point_i$, $\Qoint'_i = \Rot'_{\mathbf{x}} \Point'_i$, and convert system \eqref{eq:13_epipolar} to:
\begin{equation*}
    {\Qoint'_i}^\text{T} [\Tran']_{\times} \Rot_y(\varphi) {\Qoint'_i} = 0, \ i \in \{1,2,3\}.
\end{equation*}
This is the problem of estimating the relative pose with upright rotation from $3$ point correspondences. We solve this with the method described in \cite{DBLP:conf/3dim/SweeneyFT14}, which reduces the problem to a univariate polynomial of degree $4$. Note, that the naive approach would yield a polynomial of degree $6$. Finally, we compose $\Rot = {\Rot'}_{\mathbf{x}}^\text{T} \Rot_y(\varphi) \Rot_{\mathbf{x}}$, $\Tran = {\Rot'}_{\mathbf{x}}^\text{T} \Tran'$. 
%
%To obtain a polynomial system, we replace $\cos \varphi$, $\sin \varphi$ with $\frac{1-s^2}{1+s^2}$, $\frac{2s}{1+s^2}$, and multiply the system with $1+s^2$.
%
%The resulting system is linear in $\Tran$ elements. We can write it as
%
%\begin{equation}
%    \matr{A}(s) \Tran = 0 \label{eq:13_matrix},
%\end{equation}
%
%where the elements of $\matr{A}(s) \in \RR^{3\times3}$ depend on $s$. If \eqref{eq:13_matrix} holds, then $\matr{A}(s)$ is singular, and therefore, $\det \matr{A}(s) = 0$. This is a univariate polynomial equation of degree $6$ that can be reduced to degree $4$ \cite{DBLP:conf/eccv/FraundorferTP10}. We find $s$ with the companion matrix approach. Then, we find $\Tran$ by \eqref{eq:13_matrix}, $\Rot_y$ by \eqref{eq:13_epipolar}, and, finally, $\Rot$ by \eqref{eq:13_rot_decomposition}.

\subsubsection{Pose from 1VC and 3LCs (0-3-1)}\label{sec:031}

\noindent
Here, we discuss how to calculate the relative pose $\Rot, \Tran$ from one vanishing point correspondence and three correspondences of coplanar lines.
%
Suppose that we are given a corresponding vanishing point pair $(\Vanishing_1, \Vanishing_1')$ and three coplanar line correspondences $(\Line_1, \Line_1')$, $(\Line_2, \Line_2')$, $(\Line_3, \Line_3')$.
%
The line matches can be pairwise intersected to generate three corresponding point pairs as $\Point_i = \Line_i \times \Line_j$ and $\Point'_i = \Line'_i \times \Line'_j$, where $(i, j) \in \{(1,2), (1,3), (2,3)\}$.
%
We can use them together with the vanishing point correspondence to calculate the relative pose according to Sec.~\ref{sec:1vp3pt}.

\subsubsection{Pose from 2VCs and 2PCs (2-0-2)}\label{sec:2vp2pt}

Here, we are going to discuss, how to calculate the relative pose $\Rot$, $\Tran$ from two vanishing point and two point correspondences. This problem is overconstrained, however, removing any entity will make it underconstrained. %\PH{Acknowledge that this is actually overconstrained. Do not be very loud when doing it.}
%
Suppose that we are given two corresponding vanishing point pairs $(\Vanishing_1, \Vanishing_1')$ and $(\Vanishing_2, \Vanishing_2')$ in the two images normalized by the intrinsic camera matrices. 
Also, we are given point correspondences $(\Point_1, \Point_1')$ and $(\Point_2, \Point_2')$ both normalized by the intrinsics.

First, we calculate rotation $\Rot$ from the vanishing points. Both pairs of corresponding vanishing points are related by \eqref{eq:vanishing} which gives four systems of equations as follows:
\begin{equation}
    \begin{split}
        \Vanishing'_1 = \Rot \Vanishing_1 , \Vanishing'_2 = \Rot \Vanishing_2;
        \ \ \ \
        \Vanishing'_1 = \Rot \Vanishing_1 , -\Vanishing'_2 = \Rot \Vanishing_2;
        \\
        -\Vanishing'_1 = \Rot \Vanishing_1 , \Vanishing'_2 = \Rot \Vanishing_2;
        \
        -\Vanishing'_1 = \Rot \Vanishing_1 , -\Vanishing'_2 = \Rot \Vanishing_2. \label{eq:22_rot_4}
    \end{split}
\end{equation}
%
If $\Rot \in \text{SO}(3)$ is a valid rotation matrix, it satisfies at least one of these systems. 
Each of the systems is of form
%
\begin{equation}
    \mathbf{x}' = \Rot \mathbf{x} , \ \ \ \ \ \ \ \ \mathbf{y}' = \Rot \mathbf{y}, \label{eq:22_rot_general}
\end{equation}
%
where $\lVert \mathbf{x} \rVert = \lVert \mathbf{x'} \rVert = \lVert \mathbf{y} \rVert = \lVert \mathbf{y'} \rVert = 1$. We want to find $\Rot \in \RR^{3\times3}$ such that $\Rot^\text{T} \Rot = \textbf{I}$ and $\det \Rot = 1$.
%
If $\Rot$ is a rotation matrix, it transforms the cross product $\mathbf{x} \times \mathbf{y}$ as
%
\begin{equation}
    \Rot (\mathbf{x} \times \mathbf{y}) = \mathbf{x'} \times \mathbf{y'}. \label{eq:22_rot_cross}
\end{equation}
%
Equations \eqref{eq:22_rot_general}, \eqref{eq:22_rot_cross} together build a square system as
%
\begin{equation}
    \begin{bmatrix} \mathbf{x}' & \mathbf{y}' & \mathbf{x}' \times \mathbf{y}' \end{bmatrix} = \Rot \begin{bmatrix} \mathbf{x} & \mathbf{y} & \mathbf{x} \times \mathbf{y} \end{bmatrix}. \label{eq:22_rot_all}
\end{equation}
%
We obtain the rotation matrix $\Rot$ from \eqref{eq:22_rot_all} as:
%
\begin{equation*}
    \Rot = \begin{bmatrix} \mathbf{x}' & \mathbf{y}' & \mathbf{x}' \times \mathbf{y}' \end{bmatrix} \begin{bmatrix} \mathbf{x} & \mathbf{y} & \mathbf{x} \times \mathbf{y} \end{bmatrix}^{-1}.
\end{equation*}
%
According to \eqref{eq:22_rot_4}, we have 4 systems in form \eqref{eq:22_rot_all}. These systems yield 4 rotations $\Rot_a$, $\Rot_b$, $\Rot_c$, $\Rot_d$, each of which is consistent with the input.

For every rotation $\Rot_i, i \in \{a,b,c,d\}$, we are now going to find translation $\Tran_i$ from the two point correspondences. According to \eqref{eq:epipolar_pts}, it holds that
%
\begin{equation}
    {\Point'_1}^\text{T} [\Tran_i]_{\times} \Rot_i \Point_1 = 0, \ \ \ {\Point'_2}^\text{T} [\Tran_i]_{\times} \Rot_i \Point_2 = 0. \label{eq:22_epipolar}
\end{equation}
%
Since $\Rot_i$ is already known, 
\eqref{eq:22_epipolar} is a homogeneous linear system in the parameters of $\Tran_i$ of form
%
%\begin{equation}
    $\matr{A} \Tran_i = 0$,
%\end{equation}
%
where $\matr{A} \in \RR^{2\times3}$ is a matrix of coefficients. 
Matrix $\matr{A}$ is shown in supplementary material. 
In order to get translation $\Tran_i$, we calculate the SVD decomposition of matrix $\matr{A} = \matr{U} \matr{S} \matr{V}^\text{T}$ and take row $\matr{V}_3$ of $\matr{V}$ that corresponds to the smallest singular value.
Due to the scale ambiguity of perspective projection, $\Tran_i = \matr{V}_3$ is defined up to scale.
%
In summary, this solver yields up to four real solutions. We can determine the correct solution by checking the order of the lines, from which the VPs $\Vanishing_1$, $\Vanishing_2$ were obtained.


%\subsubsection{Pose from 1VC, 2PCs and 1LC (2-1-1$^\perp$)}\label{sec:112_orthogonal}

%\PH{We can skip this one since it has been solved. This will give us some space.}

%Here, we show how to calculate the relative pose from two point and a vanishing point correspondence, and a line correspondence orthogonal to the VP.
%
%Suppose that we are given a vanishing point match $(\Vanishing, \Vanishing')$, a line $(\Line, \Line')$ and two point correspondences $(\Point_1, \Point_1')$, $(\Point_2, \Point_2')$ in the images.
%
%Let us assume that the directions $\Dir_1$ of vanishing point $\Vanishing_1$ and $\Dir_2$ of line $\Line$ are orthogonal -- this holds similarly on their corresponding pairs in the second image. 
%
%We will use this assumption to find the vanishing point $\Vanishing_2$ in direction $\Dir_2$.

%Due to \eqref{eq:VP_calibrated}, $\Vanishing_2$ is orthogonal to $\Vanishing_1$. Since line $\Line$ has direction $\Dir_2$, $\Vanishing_2$ lies on $\Line$. 
%Therefore, it holds that
%
%\begin{equation}
%    \Vanishing_1^\text{T} \Vanishing_2 = 0 , \ \Line^\text{T} \Vanishing_2 = 0. \label{eq:12_vps}
%\end{equation}
%
%Therefore \cite{Bazin12}, we find $\Vanishing_2$ from \eqref{eq:12_vps} as
%
%\begin{equation*}
%    $\Vanishing_2 = \Vanishing_1 \times \Line$.
%\end{equation*}
%
%Analogously, we find $\Vanishing'_2$ as
%
%\begin{equation*}
%    $\Vanishing'_2 = \Vanishing'_1 \times \Line'$.
%\end{equation*}
%Now, $\Vanishing_2$, $\Vanishing'_2$ is a valid vanishing point correspondence. We can combine it with the existing correspondence $\Vanishing_1$, $\Vanishing'_1$, and with two point correspondences $(\Point_1, \Point'_1)$, $(\Point_2, \Point'_2)$, and find the relative pose as proposed in Sec.~\ref{sec:2vp2pt}.

\subsubsection{Pose from 1VC, 1PC, and 2LCs (1-2-1$^\perp$)}\label{sec:201_orthogonal}

If one of the lines $\Line_1$ is orthogonal to the direction of the vanishing point $\Vanishing_1$, and the two lines intersect as $\Point_2 = \Line_1 \times \Line_2$, we can use line $\Line_1$ as the line $\Line$ together with $\Vanishing_1$, $\Point_1$, $\Point_2$, and find the relative pose according to \cite{DBLP:conf/cvpr/ElqurshE11}.% Sec.~\ref{sec:112_orthogonal}.

\subsubsection{Pose from 1VC, and 2PC (2-0-1$^\perp$)}\label{sec:201_orthogonal_new}

If the line passing the points $\Point_1$, $\Point_2$ is orthogonal to the direction of the vanishing point $\Vanishing_1$, we can use the line $\Line = \Point_1 \times \Point_2$ together with $\Vanishing_1$, $\Point_1$, $\Point_2$, and find the relative pose according to \cite{DBLP:conf/cvpr/ElqurshE11}.

%A spcial configuration arises, when one of the lines $\Line_1$ is orthogonal to the direction of the vanishing point $\Vanishing_1$, and the two lines intersect as $\Point_2 = \Line_1 \times \Line_2$, which gives a second point correspondence. In this case, we can use line $\Line_1$ as the line $\Line$, and find the relative pose according to Sec.~\ref{sec:112_orthogonal}.

% A special configuration arises, when one of the points $\Point_1$ is obtained as a junction of two lines as $\Point_1 = \Line_1 \times \Line_2$, where the direction of line $\Line_1$ is orthogonal to the direction of the vanishing point $\Vanishing_1$. 
% In this case, we can use line $\Line_1$ as the line $\Line$, and find the relative pose according to Sec.~\ref{sec:112_orthogonal}.

%\subsection{Relative pose from single Homography (4 coplanar lines)}
%\noindent
%Here, we are going to discuss, how to calculate relative pose $\Rot$, $\Tran$ from corresponding projections of four coplanar lines into two cameras.

%Let us have projections $\Line_1, \Line_2, \Line_3, \Line_4$ of four coplanar lines into the first camera. Let us have the corresponding projections $\Line'_1, \Line'_2, \Line'_3, \Line'_4$ in the second camera. The projections are related by homography $\Hom$ %\label{eq:hom_line}:
%\begin{equation*}
%    \Line_i \sim \Hom^\text{T} \Line_i', i \in \{1,2,3,4\}.
%\end{equation*}
%This is a homogeneous linear system of 8 equations in 9 unknowns. We find homography $\Hom$ with SVD and decompose it \cite{malis:inria-00174036} into $\Hom = \Rot - \Tran \Normline^\text{T}$, which gives us the relative pose.


%\PH{Add algorithm here + some explanation and links to sections below}


%\subsection{Lines to Points}\label{sec:l2p}
%
%\noindent
%Here, we discuss how to convert line correspondences into point correspondences, which satisfy epipolar constraint \eqref{eq:epipolar_pts}.
%We use two strategies to convert line correspondences into point correspondences: 1. endpoints, 2. line junctions.
%\textbf{Endpoints} of line segments obtained by current line detectors~\cite{von2008lsd,huang2020tp,Pautrat_Lin_2021_CVPR,suarez2022elsed} are often repeatable enough, so they may be used as point correspondences.
%\textbf{Line junction} of two intersecting lines $\Worldline_1$, $\Worldline_2$ can also be used as a point correspondence. Let $\Worldpoint = \Worldline_1 \cap \Worldline_2$ be the intersection of lines $\Worldline_1$, $\Worldline_2$. Let $\Line_1, \Line_2 \in \RR^3$ be the projections of lines $\Worldline_1$, $\Worldline_2$ into camera $\Proj$. The projection $\Point \sim \Proj \Worldpoint$ of point $\Worldpoint$ is obtained as the intersection of lines $\Line_1$, $\Line_2$.
%\begin{equation*}
%    \Point = \Line_1 \times \Line_2.
%\end{equation*}

%\noindent
%Let us have two cameras $\Proj_1$, $\Proj_2$. 
%Let $\Line_1, \Line_2$ be the projections of $\Worldline_1, \Worldline_2$ into $\Proj_1$ and $\Line'_1, \Line'_2$ the projections of $\Worldline_1, \Worldline_2$ into $\Proj_2$.
%Then, the intersections $\Line_1 \times \Line_2$, $\Line'_1 \times \Line'_2$ present a valid point correspondence, and therefore, they are related by epipolar constraint \eqref{eq:epipolar_pts}. There holds:
%\begin{equation}
%    (\Line'_1 \times \Line'_2)^\text{T} [\Tran]_{\times} \Rot (\Line_1 \times \Line_2) = 0. \label{eq:epipolar}
%\end{equation}
%Equation \eqref{eq:epipolar} gives one polynomial constraint on the relative pose $\Rot, \Tran$.
%\\

%\noindent
%\textbf{Coplanar line projections} are related by the same homography $\Hom \in \RR^{3\times3}$. We are going to show that the coplanarity constraint is equivalent to the epipolar constraint on the line junction. Let $\Worldline_1$, $\Worldline_2$ be two coplanar lines. Let $\Line_1, \Line_2$ be their projections into $\Proj_1$ and $\Line'_1, \Line'_2$ their into $\Proj_2$. Then, there holds:
%\begin{equation}
%    \Line_1 \sim \Hom^\text{T} \Line'_1, \ \ \Line_2 \sim \Hom^\text{T} \Line'_2. \label{eq:same_homography}
%\end{equation}
%Because $\Proj_1$, $\Proj_2$ are calibrated, we can decompose $\Hom = \Rot - \Tran \Normline^\text{T}$ to get:
%\begin{equation}
%    \Line_1 \sim (\Rot^\text{T} - \Normline \Tran^\text{T}) \Line'_1, \ \ \Line_2 \sim (\Rot^\text{T} - \Normline \Tran^\text{T}) \Line'_2, \label{eq:homography_calibrated}
%\end{equation}
%where $\Normline$ is the normal of plane $\Plane$ defined by lines $\Line_1$, $\Line_2$. To eliminate $\Normline$, we take the cross product of \eqref{eq:homography_calibrated}.:
%\begin{equation*}
%\begin{split}
%    \Line_1 \times \Line_2 = (\Rot^\text{T} - \Normline \Tran^\text{T})^{-T} (\Line'_1 \times \Line'_2), \\
%    (\Rot - \Tran \Normline^\text{T}) (\Line_1 \times \Line_2) = (\Line'_1 \times \Line'_2).
%\end{split}
%\end{equation*}
%We multiply both sides of the equation by $[\Tran]_{\times}$ from left and use the fact that $\mathbf{x} \times \mathbf{x} = 0$ to get:
%\begin{equation*}
%     \begin{split}
%         [\Tran]_{\times} (\Rot - \Tran % \Normline^\text{T}) (\Line_1 \times \Line_2) = % [\Tran]_{\times} (\Line'_1 \times \Line'_2),
%         \\
%         ([\Tran]_{\times} \Rot - [\Tran]_{\times} \Tran % \Normline^\text{T}) (\Line_1 \times \Line_2) = % [\Tran]_{\times} (\Line'_1 \times \Line'_2),
%         \\
%         [\Tran]_{\times} \Rot (\Line_1 \times \Line_2) = % [\Tran]_{\times} (\Line'_1 \times \Line'_2).
%     \end{split}
% \end{equation*}
% Now, we multiply both sides of the equation by $(\Line'_1 % \times \Line'_2)^\text{T}$ and use the fact that % $\mathbf{y}^\text{T} (\mathbf{x} \times \mathbf{y}) = 0$ % to get:
% \begin{equation*}
% \begin{split}
%     (\Line'_1 \times \Line'_2)^\text{T} [\Tran]_{\times} % \Rot (\Line_1 \times \Line_2) = (\Line'_1 \times % \Line'_2)^\text{T} [\Tran]_{\times} (\Line'_1 \times % \Line'_2),
%     \\
%     (\Line'_1 \times \Line'_2)^\text{T} [\Tran]_{\times} % \Rot (\Line_1 \times \Line_2) = 0.
% \end{split}
% \end{equation*}
% This is exactly the epipolar constraint % \eqref{eq:epipolar}. This shows that coplanarity of lines % and the existence of the lead to the same constraint. See % Supplementary Material for a more detailed proof of % equivalence of the constraints.

%\todo{Petr: short proof of coplanar lines = junction}



==> latex/solvers_details.tex <==
\subsection{Details of the 2-0-2 Solver}
Here, we give additional details to the 2-0-2 solver, which computes the relative pose from 2 vanishing point correspondences $\Vanishing_1$, $\Vanishing'_1$, $\Vanishing_2$, $\Vanishing'_2$, and two point correspondences $\Point_1$,  $\Point'_1$,  $\Point_2$,  $\Point'_2$.

%\subsubsection{Linear system to determine translation for 2VP+2pt problem}\label{sec:2vp2pt_big_matrix}
%Here, we give the form of the $2 \times 3$ matrix $\matr{A}$ \eqref{eq:22_matrix} that is used to determine translation $\Tran$.

First, we compute rotation from the vanishing point correspondences. Because of the sign ambiguity of the vanishing point constraint, there are four rotations consistent with the input vanishing points. We denote these rotations as $\Rot_a$, $\Rot_b$, $\Rot_c$, $\Rot_d$.

After the rotations $\Rot_i, i \in \{a,b,c,d\}$ are computed from the vanishing point correspondences, we get equations:
\begin{equation*}
    {\Point'_1}^\text{T} [\Tran_i]_{\times} \Rot_i \Point_1 = 0, \ \ \ {\Point'_2}^\text{T} [\Tran_i]_{\times} \Rot_i \Point_2 = 0
\end{equation*}
This is a system of two equations whose unknowns are elements of translation vector $\Tran$. Since the system is linear and homogeneous, we can write it as:
\begin{equation*}
    \matr{A} \Tran = 0.
\end{equation*}
%\PH{We promise matrix A. Therefore, we cannot remove this part.}

%Now, we discuss notation used in \eqref{eq:matrix_202}. 
Let $t_1$, $t_2$, $t_3$ be the elements of the translation vector $\Tran = \begin{bmatrix}
    t_1 & t_2 & t_3
\end{bmatrix}^\text{T}$, let $(p'_1)_1$, $(p'_1)_2$, $(p'_1)_3$ be the elements of projection $\Point'_1 = \begin{bmatrix}
    (p'_1)_1 & (p'_1)_2 & (p'_1)_3
\end{bmatrix}^\text{T}$, and let $(p'_2)_1$, $(p'_2)_2$, $(p'_2)_3$ be the elements of projection $\Point'_2 = \begin{bmatrix}
    (p'_2)_1 & (p'_2)_2 & (p'_2)_3
\end{bmatrix}^\text{T}$. Let us write the rotation matrix $\Rot$ columnwise as:
\begin{equation*}
    \begin{bmatrix}
        \Row_1^\text{T} \\ \Row_2^\text{T} \\ \Row_3^\text{T}
    \end{bmatrix}
\end{equation*}
Using this notation, matrix $\matr{A}$ can be written elementwise as:
\begin{equation*}
\begin{split}
    \matr{A} = \begin{bmatrix}
        \matr{a}_{1,1} & \matr{a}_{1,2} & \matr{a}_{1,3}\\
        \matr{a}_{2,1} & \matr{a}_{2,2} & \matr{a}_{2,3}
    \end{bmatrix}
    \\
    \matr{a}_{1,1} = (p'_1)_3 (\Row_2^\text{T} \Point_1) - (p'_1)_2 (\Row_3^\text{T} \Point_1)\\
    \matr{a}_{1,2} = (p'_1)_1 (\Row_3^\text{T} \Point_1) - (p'_1)_3 (\Row_1^\text{T} \Point_1)\\
    \matr{a}_{1,3} = (p'_1)_2 (\Row_1^\text{T} \Point_1) - (p'_1)_1 (\Row_2^\text{T} \Point_1)\\
    \\
    \matr{a}_{2,1} = (p'_2)_3 (\Row_2^\text{T} \Point_2) - (p'_2)_2 (\Row_3^\text{T} \Point_2)\\
    \matr{a}_{2,2} = (p'_2)_1 (\Row_3^\text{T} \Point_2) - (p'_2)_3 (\Row_1^\text{T} \Point_2)\\
    \matr{a}_{2,3} = (p'_1)_2 (\Row_1^\text{T} \Point_2) - (p'_1)_1 (\Row_2^\text{T} \Point_2)\\
    %\matr{A} = \begin{bmatrix}
    %     &  & 
    %    \\
    %     &  & 
    %\end{bmatrix}
\end{split}
\end{equation*}
%Elementwise form of matrix $\matr{A}$ is given in \eqref{eq:matrix_202}.
We find translation $\Tran$ as the kernel of matrix $\matr{A}$.

==> tab_latex/full_table/7scenes.tex <==
\begin{table}%[]
    \centering
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l | ccc | c c}
        \toprule
        \multirow{2}{*}{Solver} & \multicolumn{3}{c |}{Pose Accuracy $\uparrow$} & Med.\ $\downarrow$ & Time  \\
        & AUC@5$^\circ$ & @10$^\circ$ & @20$^\circ$ & err.\ (px) & (ms) \\
        \midrule
        5PC+LO & 18.4 & 38.6 & 58.0 & \phantom{1}3.8 & \phantom{1}60 \\
        \midrule
        5-0-0~\cite{DBLP:conf/cvpr/Nister03} & 19.3 & 39.3 & 58.4 & \phantom{1}3.4 & \phantom{1}{74} \\
        4-0-0~\cite{DBLP:books/cu/HZ2004} & 21.3 & 41.6 & 59.9 & \phantom{1}3.2 & 143 \\
        0-4-0~\cite{DBLP:books/cu/HZ2004} & \phantom{1}7.1 & 19.8 & 39.2 & \phantom{1}6.5 & \phantom{1}81  \\
        3-0-1 & 12.7 & 27.8 & 44.8 & \phantom{1}5.1 & \phantom{1}77 \\
        0-3-1 & \phantom{1}9.6 & 20.7 & 34.2 & \phantom{1}7.1 & 169 \\
        2-0-2~\cite{SalaunMM16} & \phantom{1}4.5 & 11.1 & 19.8 & 20.8 & \phantom{1}\textbf{51} \\
        2-1-1$^\perp$~\cite{DBLP:conf/cvpr/ElqurshE11} & 11.3 & 25.1 & 42.5 & \phantom{1}5.6 & \phantom{1}61 \\
        1-2-1$^\perp$ & 14.5 & 33.0 & 53.3 & \phantom{1}8.4 & 161 \\
        \midrule 
        Hybrid & \textbf{22.4} & \textbf{43.6} & \textbf{62.6} & \phantom{1}\textbf{3.1} & {100} \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Relative pose estimation on 7Scenes~\cite{7scenes}.} We report the pose accuracy at $5^\circ$, $10^\circ$ and $20^\circ$, median error (px), and avg.\ time (ms) of LO-RANSAC~\cite{Lebeda2012BMVC} combined with the solver in the first column. 
    The first row (5PC+LO) gives the results of the 5-0-0 solver on SP+SG~\cite{superpoint, sarlin20superglue} matches. The next 8 rows give results of each of the solvers used within our proposed method. The last row (Hybrid) gives the result of our final approach combining all relevant solvers together using hybrid RANSAC.}
    % \caption{Rel.\ pose accuracy at $5^\circ$, $10^\circ$ and $20^\circ$, median error (px), and avg.\ time (ms) on 1610 pairs from the 7Scenes dataset~\cite{7scenes} of LO-RANSAC~\cite{Lebeda2012BMVC} combined with the solver in the first column. 
    % The first row is the results of the 5-0-0 solver on SP+SG~\cite{sarlin20superglue} matches.
    % The last one shows the results of our hybrid RANSAC.}
    \label{tab:7scenes}
\end{table}


==> tab_latex/full_table/eth3d.tex <==
\begin{table}%[]
    \centering
    \setlength{\tabcolsep}{4pt}
   \begin{tabular}{l | ccc | c c }
        \toprule
        \multirow{2}{*}{Solver} & \multicolumn{3}{c |}{Pose Accuracy $\uparrow$} & Med.\  $\downarrow$  & Time  \\
        & AUC@5$^\circ$ & @10$^\circ$ & @20$^\circ$ & err.\ (px) & (ms) \\
        \midrule
        5PC+LO & 69.5 & 78.7 & 84.4 & \phantom{1}0.8 & 210 \\
        \midrule
        5-0-0~\cite{DBLP:conf/cvpr/Nister03} & 69.7 & 78.8 & 84.4 & \phantom{1}0.8 & \phantom{1}\textbf{70} \\
        4-0-0~\cite{DBLP:books/cu/HZ2004} & 68.5 & 77.3 & 83.1 & \phantom{1}0.8 & 215 \\
        0-4-0~\cite{DBLP:books/cu/HZ2004} & 35.7 & 54.0 & 69.8 & \phantom{1}3.3 & 209 \\
        3-0-1 & 59.4 & 69.1 & 75.8 & \phantom{1}1.1 & 142 \\
        0-3-1 & 42.2 & 53.3 & 61.9 & \phantom{1}2.5 & 466 \\
        2-0-2~\cite{SalaunMM16} & 35.6 & 42.8 & 48.5 & \phantom{1}7.1 & 119 \\
        2-1-1$^\perp$~\cite{DBLP:conf/cvpr/ElqurshE11} & 48.4 & 57.4 & 64.3 & \phantom{1}1.8 & 164 \\
        1-2-1$^\perp$ & 49.2 & 58.4 & 65.1 & \phantom{1}1.7 & {145} \\
        \midrule 
        Hybrid & \textbf{72.5} & \textbf{80.6} & \textbf{85.5} & \phantom{1}\textbf{0.6} & 362 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Relative pose estimation on ETH3D~\cite{Schops_2017_eth3d}.}  We report the pose accuracy at $5^\circ$, $10^\circ$ and $20^\circ$, median error (px), and avg.\ time (ms) of LO-RANSAC~\cite{Lebeda2012BMVC} combined with the solver in the first column. 
    The first row (5PC+LO) gives the results of the 5-0-0 solver on SP+SG~\cite{superpoint, sarlin20superglue} matches. The next 8 rows give results of each of the solvers used within our proposed method. The last row (Hybrid) gives the result of our final approach combining all relevant solvers together using hybrid RANSAC.}
    % \caption{Rel.\ pose accuracy at $5^\circ$, $10^\circ$ and $20^\circ$, median error (px), and avg.\ time (ms) on 1969 pairs from the ETH3D dataset~\cite{Schops_2017_eth3d} of LO-RANSAC~\cite{Lebeda2012BMVC} combined with different solvers.
    % The 1st row is the results of the 5-0-0 solver on SP+SG~\cite{sarlin20superglue} matches.
    % The last one shows the results of the proposed hybrid RANSAC.}
    \label{tab:eth3d}
\end{table}



==> tab_latex/full_table/phototourism.tex <==
\begin{table}%[]
    \centering
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l | ccc | c c }
        \toprule
        \multirow{2}{*}{Solver} & \multicolumn{3}{c |}{Pose Accuracy $\uparrow$} & Med.\ $\downarrow$ & Time  \\
        & AUC@5$^\circ$ & @10$^\circ$ & @20$^\circ$ & err.\ (px) & (ms) \\
        \midrule
        5PC+LO & 56.5 & 70.4 & 85.3 & \phantom{1}1.4 & 186 \\
        \midrule
        5-0-0~\cite{DBLP:conf/cvpr/Nister03} & 62.0 & 75.3 & 85.2 & \phantom{1}1.4 & 169 \\
        4-0-0~\cite{DBLP:books/cu/HZ2004} & 56.5 & 70.4 & 81.3 & \phantom{1}1.6 & 164 \\
        0-4-0~\cite{DBLP:books/cu/HZ2004} & \phantom{1}9.5 & 23.9 & 44.8 & 10.0 & 194 \\
        3-0-1 & 12.0 & 22.4 & 36.5 & 15.1 & 147 \\
        0-3-1 & \phantom{1}8.7 & 17.9 & 29.3 & 24.0 & 275 \\
        2-0-2~\cite{SalaunMM16} & \phantom{1}3.7 & \phantom{1}7.8 & 13.8 & 70.5 & 109 \\
        2-1-1$^\perp$~\cite{DBLP:conf/cvpr/ElqurshE11} & 12.0 & 21.6 & 32.4 & 21.8 & \textbf{100} \\
        1-2-1$^\perp$ & 14.8 & 23.3 & 34.0 & 20.7 & \phantom{1}97 \\
        \midrule 
        Hybrid & \textbf{64.0} & \textbf{76.9} & \textbf{86.5} & \phantom{1}\textbf{1.3} & 389 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Relative pose estimation on PhotoTourism~\cite{Jin2020}.} We report the pose accuracy at $5^\circ$, $10^\circ$ and $20^\circ$, median error (px), and avg.\ time (ms) of LO-RANSAC~\cite{Lebeda2012BMVC} combined with the solver in the first column. 
    The first row (5PC+LO) gives the results of the 5-0-0 solver on SP+SG~\cite{superpoint, sarlin20superglue} matches. The next 8 rows give results of each of the solvers used within our proposed method. The last row (Hybrid) gives the result of our final approach combining all relevant solvers together using hybrid RANSAC.}
    % \caption{Relative pose AUC score at $5^\circ$, $10^\circ$ and $20^\circ$, med.\ error, and avg.\ time on 9900 pairs from the PhotoTourism dataset~\cite{Jin2020} of LO-RANSAC~\cite{Lebeda2012BMVC} combined with different solvers. 
    % The first row is the results of the 5-0-0 solver on SP+SG~\cite{sarlin20superglue} matches.
    % The last one shows the results of the proposed hybrid RANSAC.}
    \label{tab:phototourism}
\end{table}


==> tab_latex/full_table/scannet.tex <==
\begin{table}%[]
    \centering
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l | ccc | c c }
        \toprule
        \multirow{2}{*}{Solver} & \multicolumn{3}{c |}{Pose Accuracy $\uparrow$} & Med.\  $\downarrow$  & Time  \\
        & AUC@5$^\circ$ & @10$^\circ$ & @20$^\circ$ & err.\ (px) & (ms) \\
        \midrule
        5PC+LO & 17.3 & 33.9 & 50.9 & \phantom{1}6.5 & \phantom{1}\textbf{68} \\
        \midrule
        5-0-0~\cite{DBLP:conf/cvpr/Nister03} & 18.4 & 34.9 & 51.3 & \phantom{1}6.5 & {109}  \\
        4-0-0~\cite{DBLP:books/cu/HZ2004} & 18.2 & 34.2 & 50.0 & \phantom{1}7.2 & 165 \\
        0-4-0~\cite{DBLP:books/cu/HZ2004} & 10.3 & 21.2 & 34.4 & 16.2 & \phantom{1}91 \\
        3-0-1 & \phantom{1}6.8 & 16.1 & 28.7 & 11.0 & \phantom{1}94 \\
        0-3-1 & \phantom{1}2.7 & \phantom{1}7.3 & 14.1 & 52.0 & 186 \\
        2-0-2~\cite{SalaunMM16} & \phantom{1}2.8 & \phantom{1}6.2 & 11.8 & 27.5 & \phantom{1}73 \\
        2-1-1$^\perp$~\cite{DBLP:conf/cvpr/ElqurshE11} & \phantom{1}5.8 & 13.2 & 22.5 & 49.3 & \phantom{1}70 \\
        1-2-1$^\perp$ & \phantom{1}5.8 & 13.4 & 23.7 & 32.4 & 371 \\
        \midrule 
        Hybrid & \textbf{20.0} & \textbf{37.1} & \textbf{53.8} & \phantom{1}\textbf{6.4} & 151 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Relative pose estimation on ScanNet~\cite{dai2017scannet}.}  We report the pose accuracy at $5^\circ$, $10^\circ$ and $20^\circ$, median error (px), and avg.\ time (ms) of LO-RANSAC~\cite{Lebeda2012BMVC} combined with the solver in the first column. 
    The first row (5PC+LO) gives the results of the 5-0-0 solver on SP+SG~\cite{superpoint, sarlin20superglue} matches. The next 8 rows give results of each of the solvers used within our proposed method. The last row (Hybrid) gives the result of our final approach combining all relevant solvers together using hybrid RANSAC.}
    % \caption{Relative pose AUC score at $5^\circ$, $10^\circ$ and $20^\circ$, med.\ error, and avg.\ time on 1500 pairs from the ScanNet dataset~\cite{dai2017scannet} of LO-RANSAC~\cite{Lebeda2012BMVC} combined with different solvers.
    % The first row is the results of the 5-0-0 solver on SP+SG~\cite{sarlin20superglue} matches.
    % The last one shows the results of the proposed hybrid RANSAC.}
    \label{tab:scannet}
\end{table}

